Sparse Channel Reconstruction With Nonconvex Regularizer via DC Programming for Massive MIMO Systems

Sparse channel estimation for massive multiple-input multiple-output systems has drawn much attention in recent years. The required pilots are substantially reduced when the sparse channel state vectors can be reconstructed from a few numbers of measurements. A popular approach for sparse reconstruction is to solve the least-squares problem with a convex regularization. However, the convex regularizer is either too loose to force sparsity or lead to biased estimation. In this paper, the sparse channel reconstruction is solved by minimizing the least-squares objective with a nonconvex regularizer, which can exactly express the sparsity constraint and avoid introducing serious bias in the solution. A novel algorithm is proposed for solving the resulting nonconvex optimization via the difference of convex functions programming and the gradient projection descent. Simulation results show that the proposed algorithm is fast and accurate, and it outperforms the existing sparse recovery algorithms in terms of reconstruction errors.

==> dc_alg_conf.tex <==
\subsection{Alternative DC formulation and double-layer loop proximal method}
	 To solve the problem \eqref{dc_penalty_function}, we first regard the objective function as the difference of the two convex functions of $f(\mathbf x)$ and $g(\mathbf x)$ which is
	\begin{IEEEeqnarray*}{lCl}	
	 \label{dc_diff}
	 \mathop{\text{min}}\limits_{\mathbf{x}} 
	 \quad F(\mathbf x) :=  \underbrace{\frac{1}{2}\norm{\mathbf{y}-\mathbf{\Phi}\mathbf{x}}_2^2 + \lambda \norm{\mathbf x}_1}_{f(\mathbf x)} - \underbrace{\lambda \normmm{\mathbf x}_k}_{g(\mathbf x) }.
	 \IEEEyesnumber
	\end{IEEEeqnarray*} 
	 Next, we linearize the concave part $-g(\mathbf x)= - \lambda \normmm{\mathbf x}_k$ in \eqref{dc_diff} by $- \mathbf x^T \mathbf s^{t-1}$, so that at the $t$th-iteration, we solve the following convex subproblem 
	\begin{IEEEeqnarray*}{lCl}	
	 \label{dc_subp}
	 \mathop{\text{min}}\limits_{\mathbf{x}} \quad \frac{1}{2}\norm{\mathbf{y}-\mathbf{\Phi}\mathbf{x}}_2^2 + \lambda \norm{\mathbf x}_1 - \mathbf x^T \mathbf s^{t-1}
	\IEEEyesnumber
	\end{IEEEeqnarray*} 
where $\mathbf s^{t-1}$ denotes a subgradient of $g(\mathbf x)$ at $\mathbf x^{t-1}$, that is
	\begin{IEEEeqnarray*}{lCl}	
	\mathbf s^{t-1} \in \lambda \partial \normmm{\mathbf x^{t-1}}_k
	\IEEEyesnumber
	\end{IEEEeqnarray*} 
	where the subgradient $\partial \normmm{\mathbf x^{t-1}}_k$ of $\normmm{\mathbf x}_k$ at $\mathbf x^{t-1}$ is defined as \cite{Gotoh2018DC}
	\begin{IEEEeqnarray*}{lCl}	
	\partial \normmm{\mathbf x^{t-1}}_k = \mathop{\text{argmax}}_\mathbf s \left\lbrace \sum_{i=1} ^{N} x_i^{t-1} s_i \Big\vert \sum_{i=1}^N |s_i| =k , k \in [-1, 1]\right\rbrace. \\
	\IEEEyesnumber
	\end{IEEEeqnarray*} 
	A subgradient $\mathbf s \in \partial \normmm{\mathbf x^{t-1}}_k$ can be simply obtained by assigning the sign of the first $k$ largest elements of $\mathbf{x}^{t-1}$ to the corresponding elements of $\mathbf s$, i.e.,	$s_{(i)}=\sign(x_{(i)}^{t-1})$, then set the other elements of $\mathbf s$ to be zeros.
	
The algorithm framework of the proposed DC algorithm for sparse reconstruction is outlined as follows:
	\begin{itemize}
	\item[1.] \textbf{Start:} Given a starting point $\mathbf x ^0$, and a small threashold parameter $\epsilon>0$.
	\item[2.] \textbf{Repeat:} For t=1,2,... \\ 
					\hspace*{4mm} Select a subgradient $\mathbf s^{t-1} \in \lambda \partial \normmm{\mathbf x^{t-1}}_k$\\
					\hspace*{4mm} Solve the convex subproblem \eqref{dc_subp} to obtain $\mathbf x^t$\\
					\hspace*{4mm} Increment t
	\item[3.] \textbf{End:} Until $|F(\mathbf x^{t-1})- F(\mathbf x^t)|\le \epsilon$ satisfies.				
	\end{itemize}

	In Algorithm 1, at each step iteration we solve the convex subproblem \eqref{dc_subp}, which is 
	\begin{IEEEeqnarray*}{lCl}
	\label{dc_subp2}
	 \mathop{\text{min}}\limits_{\mathbf{x}} \quad 
	 \underbrace{\frac{1}{2}\norm{\mathbf{y}-\mathbf{\Phi}\mathbf{x}}_2^2 - \mathbf x^T \mathbf s^{t-1}}_{h(\mathbf x)} + \lambda \norm{\mathbf x}_1 
	\IEEEyesnumber  
	\end{IEEEeqnarray*} 
	As a $\ell_1$-regularized non-smooth convex optimization problem, \eqref{dc_subp2} can be effectively solved by the proximal gradient method.			
	At the $(k+1)$th iteration of a proximal method, the optimal point is found by minimizing the second-order approximation of the objective function of the subproblem $\eqref{sub_pro2}$, that is 
	\begin{IEEEeqnarray*}{lCl}
	\label{proximal_approximation}
	\mathop{\text{argmin}}_{\mathbf x}  \lbrace
	h(\mathbf x_k) + \triangledown h(\mathbf x_k)^T (\mathbf x- \mathbf x_k)  
	 + \frac{L_h}{2} \norm{\mathbf x- \mathbf x_k}_2^2 + \lambda \norm{\mathbf x}_1 \rbrace \\
		\IEEEyesnumber  
	\end{IEEEeqnarray*} 
	where $L_h$ should be the upper bound of the Lipshitz constant of $\triangledown h$.	
	Using the simple algebra and removing the terms independent with $\mathbf x$, it can be shown that the problem \eqref{proximal_approximation} is equivalent to the following proximal problem as
	\begin{IEEEeqnarray*}{lCl}
	\label{proximal_problem}
	\mathop{\text{argmin}}_{\mathbf x}  \lbrace
	\frac{1}{2} \norm{\mathbf x- 
	\underbrace{(\mathbf x_k - \frac{1}{L_h}\triangledown h(\mathbf x_k))}_{G(\mathbf x)}
	}_2^2 + \frac{1}{L_h} \lambda \norm{\mathbf{x}}_1\rbrace.
	\IEEEyesnumber  
	\end{IEEEeqnarray*} 
By denoting,
	\begin{IEEEeqnarray*}{lCl}
	\label{proximal_denote}
	G(\mathbf x_k) &&= \mathbf x_k - \frac{1}{L_h}\triangledown h(\mathbf x_k)\\
						&&=\mathbf x_k + \frac{1}{L_h}\left( \mathbf \Phi ^T \mathbf y - \mathbf \Phi^T \mathbf \Phi \mathbf x_k + \mathbf{s}^{t-1} \right).
	\IEEEyesnumber  
	\end{IEEEeqnarray*} 
The problem 		
	\eqref{proximal_problem} can be represented as 
	\begin{IEEEeqnarray*}{lCl}
	\label{proximal_representation}
	\mathbf x^{k+1} = \text{Prox}_{\frac{\lambda}{L_h}\norm{\cdot}_1}(G(\mathbf x_k)).
	\IEEEyesnumber
	\end{IEEEeqnarray*}
where the $\text{Prox}_{\norm{\cdot}_{\ell_1}}$ represents the proximal operator associated with the $\ell_1$ regularizer, which is given by the element-wise soft-threshold operation as
	\begin{IEEEeqnarray*}{lCl}
	\label{soft_threshold_iter}
	x_i^{k+1} &=& {\text{Prox}_{\frac{\lambda}{L_h}\norm{\cdot}_1} (G(\mathbf x_k)_i)} \\
	&=& {S(G(\mathbf x_k)_i, \lambda /{L_h} )}
	\IEEEyesnumber
	\end{IEEEeqnarray*}
where the subscript $i$ denotes the $i$th elements of a vector, and $S(\cdot, \cdot)$ denotes the soft-thresholding function and is defined as $S(a, \lambda) = \sign(a) \cdot \max(|a|- \lambda, 0)$.
When the iteration \eqref{soft_threshold_iter} terminates and the obtained optimal solution $\mathbf x^*$ will be the solution $\mathbf x^t$ for the $t$th outer iteration.

To summarize, Algorithm 1 outlines the proposed DC proximal algorithm for sparse reconstruction. 





	


